Efficient Contrastive Explanations on Demand

Recent work revealed a tight connection between adversarial robustness and restricted forms of symbolic explanations, namely distance-based (formal) explanations. This connection is significant because it represents a first step towards making the computation of symbolic explanations as efficient as deciding the existence of adversarial examples, especially for highly complex machine learning (ML) models. However, a major performance bottleneck remains, because of the very large number of features that ML models may possess, in particular for deep neural networks. This paper proposes novel algorithms to compute the so-called contrastive explanations for ML models with a large number of features, by leveraging on adversarial robustness. Furthermore, the paper also proposes novel algorithms for listing explanations and finding smallest contrastive explanations. The experimental results demonstrate the performance gains achieved by the novel algorithms proposed in this paper.

==> algs/findcxp_del.tex <==
\begin{flushleft}
  \hspace*{\algorithmicindent}
  \textbf{Input}: {
    Arguments: %Distance
    $\epsilon$;
    Parameters: %Explanation problem
    $\fml{E}$,
    %ML model $\fml{M}$, %=(\fml{F},\mbb{F},\mbb{D},\kappa)$,
    %Instance $(\mbf{v},c)$,
    %Norm
    $p$}\\
  %Theory $\fml{T}$, Features $\fml{F}$, Classifier $\kappa$, instance
  %$\mbf{v}$}\\
  \hspace*{\algorithmicindent}
  \textbf{Output}: {One CXp $\fml{S}$}
  %
\end{flushleft}

\begin{algorithmic}[1]
  \Function{$\findcxpdel$}{$\epsilon;\fml{E},p$}
  %\fml{M}=(\fml{F},\mbb{D},\mbb{F},\fml{K},\kappa),(\mbf{v},c),
  \State{$\fml{S}\gets\fml{F}$}
  \Comment{Initially, no feature is fixed}
  \For{$i\in\fml{F}$}
  \State{$\fml{S}\gets\fml{S}\setminus\{i\}$}
  %\While{$|\fml{S}|>0$}
  %\State{$i\gets\msf{RemoveFeature}(\fml{S})$}
  %\State{$\outc=\robt(\epsilon,\fml{S};\fml{M},(\mbf{v},c),p)$}
  %$\robt(\fml{W}\setminus\{i\}; \fml{T},\fml{F},\kappa,\mbf{v})$
  \State{$\outc=\robt(\epsilon,\fml{F}\setminus\fml{S};\fml{E},p)$}
  \If{\tbf{not}~$\outc$}
  \State{$\fml{S}\gets\fml{S}\cup\{i\}$}
  %\State{$\msf{InsertFeature}(\fml{S},i)$}
  \EndIf
  %\EndWhile
  \EndFor
  \State{\tbf{return} $\fml{S}$}
  %\Comment{Features in $\fml{S}$ are sufficient for changing the prediction}
  \Comment{$\fml{S}$ suffices for changing prediction}
  \EndFunction
\end{algorithmic}

